Calibrate-Extrapolate: Rethinking Prevalence Estimation with Black Box Classifiers

In computational social science, researchers often use a pre-trained, black box classifier to estimate the frequency of each class in unlabeled datasets. A variety of prevalence estimation techniques have been developed in the literature, each yielding an unbiased estimate if certain stability assumption holds. This work introduces a framework to rethink the prevalence estimation process as calibrating the classifier outputs against ground truth labels to obtain the joint distribution of a base dataset and then extrapolating to the joint distribution of a target dataset. We call this framework "Calibrate-Extrapolate". It clarifies what stability assumptions must hold for a prevalence estimation technique to yield accurate estimates. In the calibration phase, the techniques assume only a stable calibration curve between a calibration dataset and the full base dataset. This allows for the classifier outputs to be used for disproportionate random sampling, thus improving the efficiency of calibration. In the extrapolation phase, some techniques assume a stable calibration curve while some assume stable class-conditional densities. We discuss the stability assumptions from a causal perspective. By specifying base and target joint distributions, we can generate simulated datasets, as a way to build intuitions about the impacts of assumption violations. This also leads to a better understanding of how the classifier's predictive power affects the accuracy of prevalence estimates: the greater the predictive power, the lower the sensitivity to violations of stability assumptions in the extrapolation phase. We illustrate the framework with an application that estimates the prevalence of toxic comments on news topics over time on Reddit, Twitter/X, and YouTube, using Jigsaw's Perspective API as a black box classifier. Finally, we summarize several practical advice for prevalence estimation.

==> icwsm_checklist.tex <==
\section*{Paper Checklist to be included in your paper}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerTODO{Yes}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerTODO{Yes}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerTODO{Yes}
  \item Did you describe the limitations of your work?
    \answerTODO{Yes}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{Our paper is more of a methodological paper.}
      \item Did you discuss any potential misuse of your work?
    \answerTODO{Yes, we discussed different ways to select stability assumptions and the robust to the violations of wrong assumptions.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerTODO{All code used for this work will be made public for finding reproduction upon acceptance. The experiments in \Cref{sec:impacts} involve simulated data and do no raise any ethical considerations.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{Yes}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerTODO{N/A}
  \item Have you provided justifications for all theoretical results?
    \answerTODO{N/A}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerTODO{N/A}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerTODO{N/A}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerTODO{N/A}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerTODO{N/A}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerTODO{N/A}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{Yes, see our Section 2}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{Yes, see our Section 2}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{All code used for this work will be made public for finding reproduction upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{We did not train any classifers in this work.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{Yes we reported 95\% CIs.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{N/A}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerTODO{Yes}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerTODO{Our entire paper is about this. We introduce a framework to rethink the model error profile as modeling the joint distribution, which naturally captures the misclassification.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{Yes}
  \item Did you mention the license of the assets?
    \answerTODO{No}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerTODO{All code used for this work will be made public for finding reproduction upon acceptance.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{MTurk workers must consent to participate in our annotation task.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{All comments that were collected from social media sites were publicly visible and presumably intended originally for viewing by an unbounded audience. The comment collection process respected the deletion of comments.}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR (see \citet{fair})?
\answerTODO{N/A, no new datasets.}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset (see \citet{gebru2021datasheets})? 
\answerTODO{N/A}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerTODO{Yes. We listed the instructions in Section 5.1.}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerTODO{The data collection plan was submitted to the University IRB and determined to be exempt.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{Yes. The comment labeling process provided above average compensation (above U.S. minimum wage levels) to Amazon Mechanical Turkers. Workers were fully informed about their tasks prior to engaging them and no deception was involved. Workers were exposed to some offensive comments that they would not otherwise have seen, but the exposure was limited to at most 100 comments.}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerTODO{No new datasets will be released.}
\end{enumerate}

\end{enumerate}
